The BLA Benchmark: Investigating Basic Language Abilities of Pre-Trained Multimodal Models

Despite the impressive performance achieved by pre-trained language-and-vision models in downstream tasks, it remains an open question whether this reflects a proper understanding of image-text interaction. In this work, we explore to what extent they handle basic linguistic constructions -- active-passive voice, coordination, and relative clauses -- that even preschool children can typically master. We present BLA, a novel, automatically constructed benchmark to evaluate multimodal models on these Basic Language Abilities. We show that different types of Transformer-based systems, such as CLIP, ViLBERT, and BLIP2, generally struggle with BLA in a zero-shot setting, in line with previous findings. Our experiments, in particular, show that most of the tested models only marginally benefit when fine-tuned or prompted with construction-specific samples. Yet, the generative BLIP2 shows promising trends, especially in an in-context learning setting. This opens the door to using BLA not only as an evaluation benchmark but also to improve models' basic language abilities.

==> figures/bla_example_cp.tex <==
\begin{figure}[t!]
% \begin{SCfigure}

\captionsetup[subfigure]{slc=off,margin={0.2 cm,0cm}}
   \parbox[c]{0.48\columnwidth}{\includegraphics[width=\hsize]{images/ap.png}}%
  \parbox[c]{0.485\columnwidth}{
  
 \captionsetup{font=footnotesize}
  \subcaption*{Active-Passive voice \\
  \textbf{T:}
             the \textcolor{magenta} {woman} \textcolor{blue}{feeds} the \textcolor{teal} {man}. \\ 
 \textbf{T:}
		the \textcolor{teal}{man} is \textcolor{blue} {fed} by the \textcolor{magenta}{woman}. \\ 
  \textbf{F:} 
		 the \textcolor{magenta}{man} \textcolor{blue}{feeds} the \textcolor{teal}{woman}. \\
   \textbf{F:}
		the \textcolor{teal}{woman} is \textcolor{blue}{fed} by the \textcolor{magenta}{man}.}}
  

  \parbox[c]{0.48\columnwidth}{\includegraphics[width=\hsize]{images/coord.png}}%
  \parbox[c]{0.48\columnwidth}{
  \captionsetup{font=footnotesize}
  \subcaption*{Coordination \\ 
  \textbf{T:}
            the \textcolor{magenta}{man} \textcolor{blue}{wears a wetsuit} and  \textcolor{teal}{carries a surfboard.} \\ \textbf{T:}
            the \textcolor{magenta}{woman} \textcolor{blue}{wears a red bikini} and \textcolor{teal}{rides a red bike}. \\ \textbf{F:}
            the \textcolor{magenta}{man} \textcolor{blue}{wears a wetsuit} and \textcolor{teal}{rides a red bike}. \\ \textbf{F:}
            the \textcolor{magenta}{woman} \textcolor{blue}{carries a surfboard} and \textcolor{teal}{wears a red bikini}.
            }}


  \parbox[c]{0.48\columnwidth}{\includegraphics[width=\hsize]{images/rc2.png}}%
  \parbox[c]{0.48\columnwidth}{
  \captionsetup{font=footnotesize}
  \subcaption*{
       Relative Clause\\ 
       \textbf{T:}
       the \textcolor{magenta}{man} who \textcolor{blue}{wears a gray polo} \textcolor{teal}{holds a stuffed bear}. \\ \textbf{T:}
       the \textcolor{magenta}{man} who \textcolor{blue}{wears a striped shirt} \textcolor{teal}{holds a cow}. \\ \textbf{F:}
       the \textcolor{magenta}{man} who \textcolor{blue}{wears a gray polo} \textcolor{teal}{holds a cow}. \\ \textbf{F:}
       the \textcolor{magenta}{man} who \textcolor{blue}{wears a striped shirt} \textcolor{teal}{holds a stuffed bear}.
  }}
  
    \caption{One example for each of the linguistic constructions included in the benchmark. Sentences in each BLA dataset (both \textbf{T}rue and \textbf{F}alse ones) share the same template, with 3 slots being filled by as many arguments (NPs, predicates, or clauses), that we signal with different colors. E.g., in the active-passive construction, the bits in red and green are the subject and object of the sentence, respectively, while the blue bit is the predicate.
    % We use different colors to signal the different parts of the sentence\dots  \san{We need some more details in the caption to explain what the colors stand for in the sentences}
        % \san{I wonder if the tables with the templates can be merged with this example, so as to have just one figure showing the sentences and the templates used to construct them. For sure, we cannot afford the three tables in the main paper; either we find a way to compact this info, or move them to SM} 
        % \xinyi{I would prefer to put the three template table to appendix}
        }
    \label{fig:bla_example}
\end{figure}
% \end{SCfigure}

==> figures/finetune_precision.tex <==
\begin{figure}[t!]
\centering
    % \begin{subfigure}[t]
        \includegraphics[width=1\columnwidth]{images/Finetune_Model_Precision.pdf}
        
    % \end{subfigure}
\caption{Model precision comparison between zero-shot and task-specific learning on BLA tasks. Also, percision > precision. Maybe move this plot to Appendix} }
    \label{fig:finetune-model-precision-results}
\end{figure}

==> figures/zero-shot_model_performance.tex <==
\begin{figure}[t!]
\centering
    % \begin{subfigure}[t]
        \includegraphics[width=1\columnwidth]{images/Zero-shot_Model_Performance.pdf}
        
    % \end{subfigure}
\caption{Zero-shot model performance on BLA tasks.}
    \label{fig:zero-shot-model-results}
\end{figure}

==> sections/bla_dataset.tex <==
\section{The Basic Language Abilities (BLA) Benchmark} \label{sec:bla_dataset}




In this section, we describe our Basic Language Abilities (BLA) benchmark. %In Section~\ref{sec:ling-abilities}, we briefly describe the 3 investigated linguistic constructions; in Section~\ref{sec:format}, we introduce the setup and format of the benchmark; in Section~\ref{sec:construction}, we describe its automatic construction and validation.




% \subsection{Language Abilities}
\subsection{Linguistic Constructions}\label{sec:ling-abilities}


% Explain why we focus on these tasks (the colorbook task for children language abilities understanding)

% Explain the selected language phenomena (inspiration), and motivation on why, also the task setup 

% The active-passive task can test whether one can comprehend two sentences that have the same meaning but are phrased differently. The coordination and relative clause tasks assess one’s ability in understanding how different parts of a sentence are composed together into a whole. 

% \subsection{Task setup}
% The four sentences are designed to evaluate three specific language phenomena. In general,
% we avoid the use of reasoning abilities to finish our tasks by discarding descriptions related to
% reasoning tasks like numbers or positions in the construction process. To force the models to respect
% sentence-level semantics instead of relying on object recognition, we design the foils
% that only contain objects that are present in the image. Models must understand the language
% phenomena to make completely correct predictions on each caption set.



% Inspired by children’s language comprehension tasks proposed by the Coloring Book \citep{pinto2019coloring}, we investigate whether models can understand specific language phenomena to test their language comprehension abilities. The language phenomena selected from the coloring book are active-passive voices and coordination. Relative clause, another basic and important construct of the English language, is also added to our test tasks. \citet{pinto2019coloring, eisenberg_2002} suggest that preschool children can comprehend the three linguistic phenomena.

% We also add relative clause phenomenon, which is also commonly used to test one's English comprehension abilities. Language learners who are capable of understanding and using relative clauses can develop a good perception of different sentence structures \citep{yi2017teaching}.

% To build the Basic Language Abilities (BLA) benchmark, 
%We consider
% We focus on 
BLA includes three types of linguistic constructions: active-passive voice, coordination, and relative clauses, that we briefly describe below.


\paragraph{Active-Passive voice (AP)} Active-passive voice refers to the form of a verb indicating whether its grammatical subject is the agent %performs the action or is 
or the receiver of the action; e.g., \textit{`the monkey scratches the mouse'} or \textit{`the mouse is being scratched by the monkey'}, respectively.
Mastering active-passive voice implies being able to verify that two sentences have the same meaning, though the grammatical subject is different. 
% y are phrased differently.
% The active-passive task can test whether one can comprehend two sentences that have the same meaning but are phrased differently. Understanding the Active-Passive voice is crucial for understanding visual-linguistic semantics on "who is doing what to whom". 

\paragraph{Coordination (CO)} %Coordination is the joining of words, phrases, or clauses of the same type to give them equal emphasis and importance; e.g., \textit{the monkey and the mouse}, \textit{the monkey is red and tall}, or \textit{the monkey eats an apple and smiles}, respectively. 
% A conjunct is used to connect the two coordinators together. 
We focus on the coordination of predicates  joined together via the conjunction \textit{`and'}, e.g., \textit{`the monkey eats an apple and smiles'}. 
% Because distinguishing the different use of the coordinators and their meanings requires some extent of logical reasoning ability, we only use the conjunctive coordinator “and”, which adds two conjuncts together. 
% This task focuses on whether the model can understand how different parts of a sentence are composed together into a whole.
Mastering this type of coordination implies being able to verify that both predicates apply to the subject of the sentence.

% how different clauses are coordinated with each other to form a sentence about an 


\paragraph{Relative Clause (RC)} 
%Relative clauses are introduced by a relative pronoun and qualify an entity previously mentioned in the sentence. 
We focus on relative clauses attached to the subject of the sentence and introduced by the pronoun \textit{`who'}, e.g., \textit{`the monkey [who scratches the mouse] is tall'} (the relative clause in  brackets for clarity of illustration).  
% ideas by using pronouns that relate to something previously mentioned and allow the writer to combine two independent clauses into one sentence. 
Mastering relative clauses implies being able to verify that \textit{both} the predicate in the relative clause and in the main clause apply to the subject of the sentence.

% it also requires understanding how different parts of a sentence are composed together but involves a more complex sentence structure.

% \subsection{Task Setup}
\subsection{Benchmark Setup and Format}\label{sec:format}

%We aim at building a benchmark, BLA, to assess the basic language comprehension abilities of pre-Trained multimodal models. To do so, 
%for each of the 3 linguistic constructions under investigation, w
We construct a dataset of natural images and template-based sentences for each of the linguistic constructions: active-passive voice (AP), coordination (CO), and relative clause (RC).
Building on the FOIL~\cite{shekhar-etal-2017-foil} paradigm, we pair %. In particular,
each image %in a given dataset is paired 
with 4 automatically generated sentences, two correct ones, the \textit{targets}, and two incorrect ones, the \textit{foils}. 
%, (see the examples in Figure~\ref{fig:bla_example}).
Foil sentences are identical to target ones with respect to their format and syntactic structure, but contain a mistake that makes them %wrong 
semantically incorrect for the image. Concretely, in the false AP sentences the agent and the recipient are reversed, in the false CO sentences one of the conjuncts does not apply to the subject, and in the false RC sentences the predicate of the main clause does not apply to the subject. Figure~\ref{fig:bla_example} shows one sample per linguistic construction. 

%In particular, the mistake involves a wrong verb subject in AP foils (Figure~\ref{fig:ap}), a wrong coordinated clause for the referenced entity in C foils (Figure~\ref{fig:coord}), and a wrong relative clause for the referenced entity in RC foils (Figure~\ref{fig:rc}). 

\raq{Maybe this paragraph can be removed?}
\xinyi{This paragraph describes the challenges for the benchmark: only including items in the image (which might be illustrated in the previous description?), and the design rule matches the idea of not having reasoning abilities involved, simply achieved by avoiding the words describing such concepts.}
Since we aim at testing language comprehension abilities and not, e.g., the ability of models to spot whether an entity or attribute is or is not in the image, all the entities and attributes mentioned in both target and foil sentences are present in the image. To enforce this, we select images such that they always depict at least two human entities (whose roles in the event can purposely be swapped to create \textit{foils}) with their own attributes (which can be purposely assigned to the other entity to create \textit{foils}).
Moreover, no predicates or attributes involving spatial, numerical, or other types of reasoning are included in the sentences. \raq{in the prev sentence, I don't understand how this is ensured} In the next section, we describe how we automatically build the benchmark from existing resources. 
%language-and-vision data.

% that are highly similar to the captions but contain some mistakes in relation to the image. With the principle of evaluating basic language abilities, no cases in the BLA tasks involve spatial, numerical or other descriptions that require high-level reasoning skills for comprehension. To force the models to respect sentence-level semantics instead of relying on object recognition, the foils are constructed to only contain objects that are present in the image.



% dataset includes \textit{N} samples each comprising an image and 4 automatically generated sentences. Out of these 4 sentences, two are correct sentences and two are wrong sentences for the given image. For AP, the two correct sentences are an active and passive sentence where the entity performing the action in the image is\dots" Here is the right moment to refer to Figure 1


% \begin{itemize}
%     \item General setting: correct captions + foil, remove reasoning cases, construct foiling cases->rule: using objects in the images
%     \item construction of foiling cases of the AP, Coord and RC
% \end{itemize}

% We introduce the BLA benchmark, which focuses on basic language construct understanding 3 linguistic phenomenon understanding tasks: \acf{AP}, \acf{Coord} and \acf{RC}. Each test sample contains one image, two sentences (\textit{captions}) that correctly describe the image and two sentences (\textit{foils}) that are highly similar to the captions but contain some mistakes in relation to the image. With the principle of evaluating basic language abilities, no cases in the BLA tasks involve spatial, numerical or other descriptions that require high-level reasoning skills for comprehension. To force the models to respect sentence-level semantics instead of relying on object recognition, the foils are constructed to only contain objects that are present in the image.

% To focus on basic language understanding, we avoid the use of reasoning abilities to finish our tasks by discarding descriptions related to reasoning tasks like numbers or positions in the task design and construction process. Following similar task setups of previous work (ToDo: add citation), we design four alternative sentences for one image to test the specific abilities of the models. The four sentences contain two \textit{captions} that correctly describe the given image and two \textit{foils} that are highly similar to the captions but contain some mistakes in relation to the image. 
    
% To force the models to respect sentence-level semantics instead of relying on object recognition, we design the foils that only contain objects that are present in the image. Models must understand the language phenomena to make correct predictions on each caption set.

% The \ac{AP} task describes human interactions in a given image. The correct captions contain one sentence using active voice \ac{TA} and one using passive voice \ac{TP}. The foils are constructed by switching the action performer and receiver order in the sentence (See examples in Figure \ref{fig:ap}). The \ac{Coord} and \ac{RC} tasks apply the linguistic phenomena to describe attributes of human entities in the image. The two correct captions \ac{TP1} and \ac{TP2} describe distinct attributes of two persons in the image, while the foils \ac{FP1} and \ac{FP2} swap one attribute of the two human entities in the sentences that make them incorrect descriptions (See examples in \ref{fig:coord} and \ref{fig:rc}).

 % To test the active-passive voice understanding, we apply this language phenomenon to describe the human interactions in the image using two different phrased sentences. For example, "the man holds the baby" is the correct description of the human interaction in the image called \ac{TA}, while "the baby is held by the man" is another correct description of the image expressed in the passive voice called \ac{TP}. The foils simply switch the performer and receiver of the sentences. With the example above, the foils \ac{FA} is "the baby holds the man" and \ac{FP} is "the man is held by the baby". 
 
 % To test coordination and relative clause understanding, we apply the two language phenomena to describe the attributes of human entities in the image. To use similar settings as the \ac{AP} cases, we construct two correct descriptions of two human entities in the image. For example, "the man who wears a white shirt holds a controller" and "the woman who wears a blue shirt sits on a sofa". The man and woman are human entities in the same image while they have two unique attributes that distinguish them from any other entities in the image. The two sentences are correct descriptions of person 1 and person 2 in the image noted as \ac{TP1} and \ac{TP2}. The incorrect sentences are constructed by simply switching one feature of the two human entities. With the example above, the foils are "the man who wears a white shirt sits on a sofa" and "the woman who wears a blue shirt holds a controller", which are noted as \ac{FP1} and \ac{FP2}. We construct the sentences of the two linguistic phenomena using different templates.

\subsection{Dataset Construction}
\label{sec:construction}

% \input{tables/data_construction_template_AP}
% \input{tables/data_construction_template_Coord}
% \input{tables/data_construction_template_RC}


\raq{my version}

To generate our samples---each consisting of one image and a set of four sentences---we use Visual Genome~\cite{krishna2017visual}, a dataset of natural images densely annotated with \emph{objects} (bounding boxes around entities labeled with a WordNet synset), object \emph{attributes} (such as colour or shape) and relationships between the objects in the image (predicates with their arguments). 

Our procedure includes the following steps:

\paragraph{I. Selection of entities and predicates}
 
Firstly, we select images in Visual Genome that include at least two objects that are persons, which we verify using the WordNet synsets. For AP, we select images where the two persons are the arguments of the same transitive verb (one as the agent and the other one as the recipient).\footnote{We check whether the predicates in the \emph{relationships} field are part of the following list of transitive verbs: \url{https://englishvocabs.com/transitive-verbs/184-transitive-verbs-list-in-english/}} 
We make sure that they belong to two different types (e.g., \emph{man} and \emph{woman}) or that they at least have two distinct attributes (e.g., \emph{running man} and \emph{sitting man}) \xinyi{maybe use \emph{running man} and \emph{sitting man}? Tall and short requires comparison and reasoning} %RF: OK
For CO and RC, we select images where the two persons are the subject arguments of two unique predicates, i.e., two different predicates per person that apply only to that person \raq{maybe add an example}. Due to multiple annotations present in Visual Genome, checking whether two predicates are different is not trivial. For example, a given person may be annotated as being the subject of two predicates, \emph{'wears a t-shirt'} and \emph{`wears a shirt'} \xinyi{maybe we can use the example in Figure 1 again here: \emph{wears a gray polo} and \emph{wears a striped shirt}}. To capture the fact that these refer to the same relationship and should not be considered as different, we encode the predicates using Sentence-BERT \citep{reimers-2019-sentence-bert} and take them to be different, independent predicates only if their cosine similarity is lower than 0.8. 

\paragraph{II. Minimum object size}

Secondly, we filter out images where the persons identified in the previous step or the objects that are in a relationship with such persons are too small. We consider them too small if their size is below a certain ratio between the area of their bounding box and that of the entire image. We use a threshold of 0.1\% for persons and of 0.05\% for other objects (such as \emph{`bikini'} or \emph{`stuffed bear'}). 

\paragraph{III. Sentence construction} 

Thirdly, we construct target and foil sentences using the templates in \xinyi{refer to the appendix for the tables?} randomly filling them in with entities and predicates that met the constraints above.\footnote{We turn all verbs into 3rd person singular forms of the simple present tense using Python’s \textit{Pattern} library.} Since there may be a multitude of suitable entities and predicates per image, each image may end up being paired with more than one set of four sentences. 

\paragraph{IV. Grammar check} 

Finally, we encode each sentence with the GRUEN pre-trained model \cite{zhu2020gruen} and obtain a score that, following previous work \cite{parcalabescu2022valse}, we use as a proxy for grammar acceptability. We only keep samples where all the four sentences per image have a GRUEN score equal to or higher than 0.7; otherwise, we discard the whole sample. 

\raq{end of my version; all the stuff below can be removed.}

To generate our samples---each consisting of one image and a set of four sentences---we use Visual Genome~\cite{krishna2017visual}, a dataset of natural images densely annotated with object  (bounding boxes labelled with a WordNet synset), object attributes (such as colour or shape), and relationships between the objects in the image. \raq{refer to app if there is one with more details}
%, and use it to generate our templated target and foil sentences. 
%In particular, we consider the VG annotation fields \textit{objects} \xinyi{(annotated bounding box size and sunsets of an object)}, \textit{attributes} \xinyi{(color or shape or other attributes of an object)}, and \textit{relationships} \xinyi{(annotated subject, object and predicate for the their inteaction)} (see Appendix \ref{subsec:vg} for more details).



%Based on the setup and format described above, we devise an automatic pipeline that, for each dataset under construction, selects suitable images \xinyi{and relationship annotations} from Visual Genome and generates 4 sentences---two \textit{targets} and two \textit{foils}---embedding the investigated linguistic construction.
% Following the task setup, we construct the BLA benchmark using \ac{VG} annotation fields \textit{relationships}, \textit{attributes}, \textit{objects} and \textit{image data} (see Appendix \ref{subsec:vg} for more details). An automatic pipeline is designed to select images and generate sentences that contain specific linguistic phenomena.
Our pipeline includes the five following steps: 
%, that we describe below in the right order.


% The pipeline follows the steps \textit{Select}, \textit{Image filter}, \textit{Extract unique attributes} (only for \ac{Coord} and \ac{RC}), \textit{Sentence Construction} and \textit{}

% We make use of the \ac{VG} annotations for our dataset construction, which contain fields \textit{relationships}, \textit{attributes}, \textit{objects}, \textit{image data} and so on (see Appendix \ref{subsec:vg}). We design a semi-automatic pipeline to construct our task datasets using the following steps.

\paragraph{I. Image selection} 
% This step loops over images in Visual Genome and \xinyi{based on their \textit{relationships} annotations} selects the ones that meet the criteria in our setup, i.e., they depict at least two human entities \san{how do we check this? with WordNet as below?} \xinyi{using WordNet} and \san{their captions?} do not contain any numerical (e.g., three, many) or spatial words (e.g. left, on top of). 

This step loops over images in Visual Genome and  selects the ones that meet the criteria in our setup based on their \textit{relationships} annotations, i.e., none of the \textit{subject} annotations contain any numerical words (e.g., three, many) and at least two human entities are annotated in the \textit{relationships} by object id verification and WordNet for human-denoting word.
For AP only, we additionally filter out images whose \textit{relationships} field does not contain at least a human-denoting word---identified using WordNet \citep{10.1145/219717.219748}---labeled as \textit{subject} and one labeled as \textit{object}. Moreover, we only keep the 
\textit{relationships} whose annotated \textit{predicate} is a transitive verb, which is automatically checked based on a list of transitive verbs available online.\footnote{\url{https://englishvocabs.com/transitive-verbs/184-transitive-verbs-list-in-english/}} For C and RC only, we select images where at least two different human entities \textit{($P_1$, $P_2$)} are annotated in the \textit{relationships} field. And each entity should have at least two \textit{relationships} items that can be used to construct attributes.


% The human entity words are verified using the WordNet \citep{10.1145/219717.219748} tools. 
% In the meanwhile, rules are added to only keep the \textit{relationships} whose annotated \textit{predicate} is a transitive verb, which is automatically checked with the \textit{Transitive Verbs List in English} \footnote{\url{https://englishvocabs.com/transitive-verbs/184-transitive-verbs-list-in-english/}}. For \ac{Coord} and \ac{RC} tasks, we select images where at least two different human entities \textit{($P_1$, $P_2$)} are annotated in the \textit{relationships}. And each entity should have at least two \textit{relationships} items that can be used to construct attributes.


% we apply the extra filter that images whose \textit{relationships} contains human entity words in the \textit{subject} and \textit{object} annotations.
% potential images and annotations that would meet our task setup requirements. For all tasks, we discard cases and annotations that contain numerical and positional reasoning words (e.g. left, on top of) in this step. 
% For \ac{AP} task, we automatically select images whose \textit{relationships} contains human entity words in the \textit{subject} and \textit{object} annotations. The human entity words are verified using the WordNet \citep{10.1145/219717.219748} tools. In the meanwhile, rules are added to only keep the \textit{relationships} whose annotated \textit{predicate} is a transitive verb, which is automatically checked with the \textit{Transitive Verbs List in English} \footnote{\url{https://englishvocabs.com/transitive-verbs/184-transitive-verbs-list-in-english/}}. For \ac{Coord} and \ac{RC} tasks, we select images where at least two different human entities \textit{($P_1$, $P_2$)} are annotated in the \textit{relationships}. And each entity should have at least two \textit{relationships} items that can be used to construct attributes. 




\paragraph{II. Object size filter} This step filters out the images for which the objects in some relationship---included in the \textit{relationships} annotation---are particularly small in the context of the whole image.
We define an object as \textit{small} based on the ratio between its size in the image (the area of its bounding box) and that of the entire image. 
If the ratio is below a certain threshold, defined manually, then the image; otherwise, it is kept.\footnote{We set to 0.1\% the object/image threshold for human entities; to 0.05\% for attributes.}
Information about image and object size is extracted from the \textit{image data} and \textit{objects} annotation fields, respectively. 



% original above
% \paragraph{Image filter} This step filters images where the targeted \textit{relationships} contain too small items that are difficult to recognize for both humans and models. We calculate the object bounding box ratios of the whole image size with \textit{image data} and \textit{objects} annotations. Thresholds are manually selected to discard images and \textit{relationships} that contain subtle objects. The threshold for human entities is 0.1\% of the whole image size and 0.05\% for attributes.
% Since the \textit{relationships} contain relationships of every item in the image, some small items in the background may be selected, which is difficult to recognize for both humans and models. Therefore, relationships that contain imperceptible items are discarded. We manually select thresholds for the minimum ratio size of an item in an image, which is the bounding box taking up at least 0.1\% of the whole image size for human entities and 0.05\% for attributes.



\paragraph{III. Unique attributes extraction} In C and RC only, we ensure that the selected attributes unequivocally refer to one human entity in the image. For example, that the attribute \textit{wears a tie} only applies to one person, so as to distinguish that entity from the other(s) in the image.
To do so, we encode all attribute phrases linked to a given entity using word2vec \cite{mikolov2013distributed} and discard repeated attribute annotations. Then, we encode them using the pre-trained Sentence-BERT model \citep{reimers-2019-sentence-bert} and compare the attributes of the two human entities in the image. With this method, we construct a list of human entities with their distinct attributes.




% \paragraph{Extract unique attributes} This step only applies to \ac{Coord} and \ac{RC} constructions. It guarantees the selected attributes can distinguish two different human entities in the image. The attribute phrases are constructed using \textit{relationships} annotations. We first apply Word2Vec \citep{mikolov2013distributed} similarity to discard the repeated similar attribute annotations of the same person. Then the pretrained Sentence-BERT model \citep{reimers-2019-sentence-bert} is applied to compare the attributes of every two human entities in the image. With this method, we construct a list of human entities with their distinct attributes.

% using a similarity threshold of 0.8. For each person entity, we select a list of their unique attributes that are different from the attributes of other persons in the image.


\paragraph{IV. Templated sentence construction} For AP, we construct target and foil sentences using the template in Table \ref{tab:active-passive template}. 
To avoid ambiguity when the subject and object are annotated with the same word but indeed refer to different entities in the image (e.g. the word \textit{player} referring to two distinct players), we fill in the template not only with the noun but also their corresponding attribute. If it is a single-word attribute, we prepend it to the noun; if it is a multi-word attribute, we append it to it.
% and replace the subject and object with “distinct attribute + subject/object name” (when the attribute contains only one word) or “subject/object name + distinct attribute” (when the attribute contains more than one word). 
We turn all predicates into the simple present tense and make them agree with the subject in the number using Python’s \textit{Pattern} library.

For C and R, we construct target and foil sentences using the template in Table \ref{tab:coordination template}. Two attributes are randomly chosen from the list of unique attributes of the person and either concatenated using the conjunction \textsc{and} (C) or placed in the main and relative clause (introduced by the pronoun \textsc{who}) slots.
For each image, more than one target and foil can result from this step.





% \paragraph{Sentence Construction} For \ac{AP} task, we generate the sentences using a template (Table \ref{tab:active-passive template}). To avoid ambiguity when the subject and object are annotated using the same word but refer to different entities in the image (e.g. referring to two men), we add attributes of the persons and replace the subject and object with “distinct attribute + subject/object name” (when the attribute contains only one word) or “subject/object name + distinct attribute” (when the attribute contains more than one word). The predicate is transformed into the simple present tense and agrees with the subject in numbers using Python’s \textit{Pattern} library. 

% For \ac{Coord} and \ac{RC}, we construct the sentences using the template in Table \ref{tab:coordination template} and Table \ref{tab:relative-clause template}, where the two attributes are randomly chosen from the list of unique attributes of the person. That means, for each image, more than one set of correct captions and foils can be constructed in this step.

\paragraph{V. Grammar check} We discard sentences that are of poor quality. Concretely, we encode each sentence with the GRUEN pre-trained model \cite{zhu2020gruen} and obtain a score that, following previous work \cite{parcalabescu2022valse}, we use as a proxy for grammar acceptability. We keep sentences if their GRUEN score is equal to or higher than 0.7; otherwise, we discard them. We then pick the sentence set with the highest GRUEN score and use that one\dots

\san{In the entire pipeline description, we miss a clear intuition of the relationship between the construction of a single sentence and the package of 4 sentences that we call a sample or datapoint. For example, how many sentences (sets of sentences) are created per image? Do we first construct the target sentences, and then generate the foils accordingly? Or do we construct the 4 of them at the same time? How do the filters apply to the set, e.g., what if only one out of 4 sentences is below 0.7 in GRUEN?}
\xinyi{
in the construction process, we first extract the \textit{relationships} information which contains [subject, object, predicate] fields that meet our requirement with the steps 1, 2, 3. And we construct the 4 sentences in a datapoint using step 4 template at a time. In this case, multiple datapoint for one image might exist due to multiple \textit{relationships} might meet our requirements from the first 3 steps. When going through grammar check, if one sentence does not meet our need, we would discard the whole datapoint.
}


% \paragraph{V. Sentence filter} To ensure the language quality of the constructed sentences and to discard the extra captions of the same image, we apply GRUEN pretrained model \citep{zhu2020gruen} to discard caption sets that contain ungrammatical sentences. We discard those with a sentence GUREN score lower than 0.7 and only keep the caption set with the highest GRUEN score for each image. 



\subsection{Descriptive Statistics} In Table \ref{tab:bla_benchmark_statistics}, we report the dataset size, vocabulary size, average sentence length, average GRUEN scores, and the number of unique predicates (for AP) or distinctive attributes (for C and RC tasks). \xinyi{The difference between the statistics in C and RC is caused by the grammar checker filter, which discards more RC examples than the C ones.}

\san{Comment some of these numbers? E.g., different size, different vocabulary size, sentence length, etc.?}

% It is worth mentioning that the difference in size between C and RC---which use the same  is caused by the GRUEN score filter, where more examples in Relative Clause were discarded. 








% \subsection{Descriptive Statistics} We report the dataset size, vocabulary size, average sentence length, average GRUEN scores and the number of unique predicates (for the \ac{AP} task) or distinctive attributes (for \ac{Coord} and \ac{RC} tasks) in Table \ref{tab:bla_benchmark_statistics}. Using the same construction process, the difference in the dataset size between \ac{Coord} and \ac{RC} datasets is caused by the GRUEN score filter, where more examples in Relative Clause were discarded. 


\input{tables/bla-benchmark-statistics}
% With the steps described in Section \ref{}, we construct the \ac{BLA} datasets. Statistics contains: dataset sizes, vocabulary sizes, average sentence length, average GRUEN scores and the number of unique predicates (for the \ac{AP} task) and the number of distinctive attributes (for \ac{Coord} and \ac{RC} tasks).


==> tables/bla-benchmark-statistics.tex <==
%
\begin{table}[]
\begin{tabular}{@{} l@{} c@{} c @{} c@{}c@{}c@{}}
\toprule
 &
  \begin{tabular}[c]{@{}c@{}} \hspace{1 mm} Size \end{tabular}&
  \hspace{1.5 mm}\#Vocab. &
  \begin{tabular}[c]{@{}c@{}}Avg. \\  \hspace{1 mm} sentence \\ length\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Avg. \\ \hspace{1 mm} GRUEN \\ score\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\hspace{1 mm} \# preds/\\ attrs\end{tabular} \\ \hline
AP    & 613 & 165 & 6.33  & 0.86 & 43   \\
CO & 800 & 827 & 10.46 & 0.84 & 1670 \\
RC    & 789 & 807 & 10.46 & 0.85 & 1628 \\ \bottomrule
\end{tabular}
    \caption{Descriptive statistics of the 3 BLA datasets. AP: Active-Passive voice. CO: Cooridnation. RC: Relative Clause. 
    % The number of unique predicates is for the AP dataset and the number of distinctive attributes is for the \ac{Coord} and \ac{RC} tasks.
    }
\label{tab:bla_benchmark_statistics}
\end{table}

==> tables/data_construction_template_RC.tex <==
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ | c | c| c| } 
  \hline
   &Person & Template \\ 
  \hline
   TP$_1$ & P$_1$ &  the \textcolor{magenta}{\textit{$p_1$}} who  \textcolor{blue}{\textit{$f_{1p_1}$}}  \textcolor{teal}{\textit{$f_{2p_1}$}} \\ 
  \hline
   TP$_2$ & P$_2$ &  the \textcolor{magenta}{\textit{$p_2$}} who \textcolor{blue}{\textit{$f_{1p_2}$}} \textcolor{teal}{\textit{$f_{2p_2}$}}\\ 
  \hline
   FP$_1$ & P$_1$ &  the \textcolor{magenta}{\textit{$p_1$}} who \textcolor{blue}{\textit{$f_{1p_1}$}} \textcolor{teal}{\textit{$f_{2p_2}$} /\ \textit{$f_{1p_2}$}}\\ 
  \hline
   FP$_2$ & P$_2$ &  the \textcolor{magenta}{\textit{$p_2$}} who  \textcolor{blue}{\textit{$f_{2p_1}$}} \textcolor{teal}{\textit{$f_{1p_2}$}/\ \textit{$f_{2p_2}$}}\\ 
  \hline
\end{tabular}}
\caption{\label{tab:relative-clause template}Template for caption construction in \ac{RC} dataset. \textbf{TP$_1$.} True Person$_1$. \textbf{TP$_2$.} True Person$_2$. \textbf{FP$_1$.} False Person$_1$. \textbf{FP$_2$.} False Person. Examples: TP$_1$: the \textcolor{magenta}{man} who \textcolor{blue}{wears a white shirt} \textcolor{teal}{holds a controller}. TP$_2$:  the \textcolor{magenta}{woman} who \textcolor{blue}{wears a blue shirt} \textcolor{teal}{sits on a sofa}. FP$_1$: the \textcolor{magenta}{man} who \textcolor{blue}{wears a white shirt} \textcolor{teal}{sits on a sofa}. FP$_2$: the \textcolor{magenta}{woman} who \textcolor{blue}{holds a controller} \textcolor{teal}{wears a blue shirt}.}
\end{table}

==> tables/human_performance.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Metric                  & AP    & Coord & RC    \\ \midrule
Accuracy (\%)           & 92.00 & 90.00 & 85.00 \\
Precision\_caption (\%) & 90.00 & 79.00 & 79.00 \\
Precision\_foil (\%)    & 94.00 & 95.00 & 95.00 \\ 
Disagreement rate (\%)    & ToDO & ToDO & ToDO \\
\bottomrule
\end{tabular}
\caption{Human performance on the BLA tasks.}
\label{tab:human_performance_results}
\end{table}
